Observational Overfitting in Reinforcement Learning

A major component of overfitting in model-free reinforcement learning (RL) involves the case where the agent may mistakenly correlate reward with certain spurious features from the observations generated by the Markov Decision Process (MDP). We provide a general framework for analyzing this scenario, which we use to design multiple synthetic benchmarks from only modifying the observation space of an MDP. When an agent overfits to different observation spaces even if the underlying MDP dynamics is fixed, we term this observational overfitting. Our experiments expose intriguing properties especially with regards to implicit regularization, and also corroborate results from previous works in RL generalization and supervised learning (SL).

==> text/related_works.tex <==

\section{Related Work}
Recently, multiple works have proposed analysis on overfitting in reinforcement learning. These include, but are not limited to studying:

\begin{compactitem}
\item MDP's with changing video backgrounds \citep{videobackground}, determinism \citep{brute} in pixel-based Atari \citep{atari}, procedurally generated levels \citep{coinrun}, and domain randomization/data augmentation \citep{domain_randomization}.
\item Brittle policies \citep{robust_adversarial_rl, simplicity} in control such as Mujoco.
\item Memorization of rewards \citep{dissection} in various GridWorlds \citep{overfittingRL}, fine tuning with environments such as Gym-Retro \citep{learnfast}.
\item Theoretical ways of studying RL generalization \citep{salesforce, principle, lipschitz}
\end{compactitem}
Certain methods have risen to prevent overfitting, stemming from both theoretical analysis and empirical practice - for instance, on Lipschitz continuity of a policy \citep{lipschitz}, smoothness of training landscape due to entropy \citep{entropy_regularization}, weight regularization \citep{coinrun}. 

Other methods to assist the agent include adding supervision into the model, such as object segmentation \citep{rl_segmentation}, model-based priors \citep{}, using pretrained models \citep{}. 

In our study, we characterize the part of RL overfitting that is caused by convolutional networks and observation spaces, when training \textit{end-to-end}. Previously there have been works on understanding the decision-making of an agent through saliency and other network visualizations \citep{saliency, atari-zoo}. In our setting, we are more motivated by learning theoretic frameworks to capture this phenomena, as there is vast literature on understanding the generalization properties of SL classifiers \citep{exploring_gen, spectralrandom, sensitivity, gen_overparametrization}. We study how these topics may relate, by analyzing the observational generalization capabilities of an agent.

